Contact-aware simulations of particulate Stokesian suspensions

We present an efficient, accurate, and robust method for simulation of dense suspensions of deformable and rigid particles immersed in Stokesian fluid in two dimensions. We use a well-established boundary integral formulation for the problem as the foundation of our approach. This type of formulations, with a high-order spatial discretization and an implicit and adaptive time discretization, have been shown to be able to handle complex interactions between particles with high accuracy. Yet, for dense suspensions, very small time-steps or expensive implicit solves as well as a large number of discretization points are required to avoid non-physical contact and intersections between particles, leading to infinite forces and numerical instability. Our method maintains the accuracy of previous methods at a significantly lower cost for dense suspensions. The key idea is to ensure interference-free configuration by introducing explicit contact constraints into the system. While such constraints are unnecessary in the formulation, in the discrete form of the problem, they make it possible to eliminate catastrophic loss of accuracy by preventing contact explicitly. Introducing contact constraints results in a significant increase in stable time-step size for explicit time-stepping, and a reduction in the number of points adequate for stability.

==> archive.tex <==
\para{Literature review quotations:}
\begin{itemize}
\item To robustly avoid non-penetration, repulsive forces must be very stiff or even nonlinear. To robustly avoid non-physical jitter effects, forces must be continuous \citet{Otaduy2009}

\item The solution to our constrained dynamics problem alone does not guarantee a penetration-free state at the end of a time step. There are two possible reasons: the linearization of the contact constraints, and the fact that the collision response induced by some constraints $g$ may in turn violate other constraints that were not accounted for \citet{Otaduy2009}

\item One can check the residual of collision response \citet{Otaduy2009} during iterations to decide when to stop during an LCP solve

\item The first approach is that the force value is directly related to an interpenetration measure: This is the penalty method. The second approach, called the imposed motion method, freezes motion along the normal to all contacts.\citet{Duriez2006}

\item The principle of virtual work requires the constraint force to be orthogonal to the constraint, which means that $f=J^T \lambda$ \citet{Erleben2007}

\item \citet{Baraff1998} the usual objections to enforcing constraints with springs very stiff equations--do not carry as much weight because we're using implicit method. We tried this for a time, and found it to be a not unreasonable constraint enforcement mechanism. However, penalty methods do not enforce constraints exactly, and they do add some additional stiffness to the system.
\end{itemize}


==> makefile <==
###
## generic makefile for latex projects
## Author: Abtin Rahimian
###

###
## Plain 'make' should work most of the time, other useful patterns are
##  $ make help              #to see this
##  $ make verb              #for debugging
##  $ make nobib             #for faster compilation
##  $ make PROJ=name         #for project with different name from the dir
##  $ make OUTEXT=dvi        #for dvi output with latex compiler
##
## to have a faster compilation, this does most of passes in quiet
## mode. The downside is that it hides the error in case of
## failure. To see the error either "make verb" or "make VERB='yes'".
###

## user options
VERB	= yes
NOBIB   = no
PROJ    = ves2d_collision
LXX     = ${PDFLATEX}
OUTEXT  = pdf
SUMMARY = grep "\(error\|warn\|warning\|repeated\|skipping\)" -in --color
SYNC    = -synctex=1
ONEPASS = no
FIGRES  = 300

## programs
PDFLATEX = pdflatex
LATEX	 = latex
BIB	 = bibtex
DVI	 = dvipdf
PS	 = ps2pdf

## internal flag
QUIET	 =
LXFLAG 	 = -file-line-error -halt-on-error -shell-escape ${SYNC}
LXDFLAG  = ${LXFLAG}
BIBEXT   = bbl
INTEXT   = out

ifeq (${VERB},no)
  QUIET = -interaction=batchmode
endif

ifeq (${NOBIB},yes)
  BIBEXT = nobbl
endif

ifeq (${ONEPASS},no)
  LXFDFLAG += -draftmode
else
  INTEXT    = ${BIBEXT}
endif

TEXFILES = $(shell ls *.tex *.bib)

## project rules ##########################################################
###########################################################################
all: $(addsuffix .${OUTEXT}, ${PROJ})

## utility rules ##########################################################
###########################################################################
bib: $(addsuffix .${BIBEXT}, ${PROJ})

help:
	@head -18 ${MAKEFILE_LIST}

verb:   ## verbose make
	${MAKE} VERB=yes all

nobib:
	${MAKE} NOBIB=yes all

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4    	\
	-dPDFSETTINGS=/printer -dNOPAUSE -dQUIET -dBATCH   	\
	-dDownsampleColorImages=true			 	\
	-dDownsampleGrayImages=true 				\
	-dDownsampleMonoImages=true 				\
        -dColorImageResolution=${FIGRES}			\
        -dGrayImageResolution=${FIGRES}				\
        -dMonoImageResolution=${FIGRES}				\
	-dColorImageDownsampleThreshold=1.5 			\
	-dGrayImageDownsampleThreshold=1.5 			\
	-dMonoImageDownsampleThreshold=1.5 			\
	-sOutputFile=${PROJ}-cmprs.pdf ${PROJ}.pdf

open:
	open -a /Applications/TeX/TeXShop.app $(addsuffix .${OUTEXT}, ${PROJ})

## generic rules ##########################################################
###########################################################################
%.pdf:${TEXFILES}
	${MAKE} LXX=${PDFLATEX} $*.${INTEXT}

%.dvi:${TEXFILES}
	${MAKE} LXX=${LATEX} $*.${INTEXT}

%.out:%.tex ${TEXFILES} %.${BIBEXT}
	${LXX} ${QUIET} ${LXDFLAG} $<
	${LXX} ${QUIET} ${LXFLAG} $<
	${SUMMARY} $*.log $*.blg
	${MAKE} clean

%.aux:%.tex ${TEXFILES}
	${LXX} ${QUIET} ${LXDFLAG} $<

%.${BIBEXT}:%.aux
	-${BIB} $* 1>/dev/null
	-${SUMMARY} $*.blg

%.nobbl:%.aux
	@echo "skipping the bib make step"

clean:
	${RM} *out *-blx.bib *run.xml *.nav *.snm *.toc *.cb *.cb2 *.spl *.cpt *.tdo *.lof *.lot *.auxlock figs/*.log figs/*.spl *.upa

cleaner:
	${MAKE} clean
	${RM} *log *blg $(addsuffix .aux, ${PROJ}) $(addsuffix .synctex.gz, ${PROJ})
	${RM} figs/*.dpth figs/*.md5 figs/*.dep figs/*-converted-to.pdf figs/external-*.cb* figs/external-*.xml

cleanest:
	${MAKE} cleaner
	${RM} $(addsuffix .pdf, ${PROJ}) $(addsuffix .dvi, ${PROJ}) $(addsuffix .${OUTEXT}, ${PROJ}) $(addsuffix .bbl, ${PROJ})

distclean:
	${MAKE} cleanest
	${RM} figs/external-* figs/${PROJ}-*

.PHONY: clean cleaner cleanest distclean
.SUFFIXES:
.SECONDARY:

